Simulation of Dark Bremsstrahlung in GEANT4

A technique for the simulation of dark bremsstrahlung for electrons and muons in GEANT4 is presented. The total cross section is calculated using the Weizs\"{a}cker-Williams approximation and the outgoing kinematics are produced by scaling events produced in MadGraph/MadEvent to lower incident lepton energies, allowing the simulation to account for thick targets and lepton sources without fixed energies. Compared with dedicated samples produced at an arbitrary particle energy, typical precision of better than 5% is achieved.

==> tabs/implementation_parameteres.tex <==
\begin{table}[!htb]
    \centering
    \begin{tabular}{|c|llp{0.45\textwidth}|} 
    \hline
        Parameter & Reqd? & Level & Description \\
        \hline
        A' Mass & Yes & Process & Mass in MeV of the A' to simulate (must match mass in LHE data) \\
        \mg{} Data & Yes & Model & Path to directory containing LHE files of dark brem events to be used for the simulation. \\
        Muons & Yes & Process & \ac{db} should happen off muons (if true) or electrons (if false) \\
        Cross Section Threshold & No & Model & Minimum incident energy in GeV for cross section to be non-zero. Set to the maximum of the input threshold and twice the A' mass. (Default = twice the A' mass) \\
        Mixing Strength ($\epsilon$) & No & Model & Dark brem cross section calculation factors in the ``strength" of the dark brem mixing using $\epsilon^2$ (Default = 1.) \\
        Scaling Method & No & Model & How the model should interpret the LHE data and scale it to the actual incident energy. More detail in Appendix \ref{sec:docs:method}, options in Table~\ref{tab:scaling_methods} (Default = ``Forward Only'') \\
        Cross Section Method & No & Model & How the model should calculate the total cross section. More detail in Appendix \ref{sec:docs:xsec} (Default = Full for $1 < m_A/m_\ell < 50$ and Improved otherwise) \\
        ID of Dark Photon in LHE & No & Model & PDG ID number used for dark photon in the pass \mg{} data (Default = 622) \\
        Allow $>1$ Dark Brem & No & Process & Allow for dark brem process to occur more than once per event (i.e. \emph{don't} deactivate the process if PostStepDoIt is called --- the process is reactivated in RunManager::TerminateOneEvent). (Default = False) \\
        Cache Cross Sections & No & Process & Cache the calculated cross sections determined by the model for later use. A good amount of speed improvement is gained from this and should only be disabled if the cross section calculation is not deterministic. (Default = True) \\
        \hline
    \end{tabular}
    \caption{Parameters that can be used to configure the dark brem simulation}
    \label{tab:implementation_parameters}
\end{table}

==> tabs/scaling_methods.tex <==
\begin{table}[!htb]
    \centering
    \begin{tabular}{|c|p{0.5\textwidth}|}
        \hline
        Interpretation Method & Description
        \\ \hline
        Forward Only &
        Loops through the LHE data until $p_T^2+m_e^2$ from the LHE is less than the actual electron energy squared,  
        then uses the chosen $p_T$ with the actual total energy (choosing $p_z>0$)\\
        CM Scaling &
        Scales the LHE vertex momenta to the actual electron energy using Lorentz boosts into and out-of the Center of Momentum frame\\
        Undefined &
        Just uses the LHE data without any modification (i.e. assumes the actual electron 4-momentum is the 4-momentum in the LHE)
        \\ \hline
    \end{tabular}
    \caption{Interpretation methods for the input LHE file.}
    \label{tab:scaling_methods}
\end{table}
